A Study of the Landscape of Privacy Policies of Smart Devices

As the adoption of smart devices continues to permeate all aspects of our lives, user privacy concerns have become more pertinent than ever. Privacy policies outline the data handling practices of these devices. Prior work in the domains of websites and mobile apps has shown that privacy policies are rarely read and understood by users. In these domains, automatic analysis of privacy policies has been shown to help give users appropriate insights. However, there is a lack of such an analysis in the domain of smart device privacy policies. This paper presents a comprehensive study of the landscape of privacy policies of smart devices. We introduce a methodology that addresses the unique challenges of smart devices, by finding information about them, their manufacturers, and their privacy policies on the Web. Our methodology utilizes state-of-the-art analysis techniques to assess readability and privacy of smart device policies and compares it policies of e-commerce websites and mobile applications. Overall, we analyzed 4,556 smart devices, 2,211 manufacturers, and 819 privacy policies. Despite smart devices having access to more intrusive data about their users (using sensors such as cameras and microphones), more than 1,167 of the analyzed manufacturers did not have policies available. The study highlights that significant improvement is required on communicating the data management practices of smart devices.

==> analysis.tex <==

PrivacyLens incorporates a suite of NLP and ML techniques to perform different types of analyses and extract various insights from a privacy policy. The goal of this stage is to determine the readability of the policy document and evaluate its acceptability with respect to privacy. 


\subsection{Privacy Analysis}

\system extracts the following four privacy features of an IoT device policy.

\paragraph{Keyword Coverage and Usage.}
We utilized NLP techniques to preprocess and clean privacy policy texts from three distinct datasets: Android applications, Internet of Things (IoT) devices (categorized into those mentioning vs. not mentioning specific devices), and various websites to ensure accuracy and consistency, setting the stage for a more reliable analysis.
Our approach combined the use of seed keywords, inspired by the foundational work\cite{wilson2016creation,inproceedings_1}, with the addition of two categories: one dedicated to IoT-related data practices\cite{9581254} and the other focused on legal compliance aspects, particularly with legislation such as GDPR and CCPA (see~\Cref{tab:privacy_keywords}). 
To delve deeper into the thematic structure of these privacy policies, we employed Latent Dirichlet Allocation (LDA) for topic modelling across all three datasets not only facilitating the extraction of underlying topics but also enabling us to compare the coverage of seed keywords in privacy policies across different datasets, yielding insights into their similarities and distinctions.
For a quantitative assessment of keyword usage, we utilized sklearn's CountVectorizer tool\footnote{\url{https://scikit-learn.org/stable/modules/generated/sklearn.feature_extraction.text.CountVectorizer.html}}, which was instrumental in calculating the frequency of our expanded set of seed keywords within each dataset. By doing so, we were able to conduct a systematic and comparative analysis of keyword prevalence and relevance across the various categories of privacy policies, offering a nuanced understanding of the focus in these documents.
\begin{table*}[!htb]
\centering
%\small
\footnotesize
\begin{tabularx}{\textwidth}{|p{2.8cm}|X|p{6cm}|}
\hline
\textbf{Privacy Attribute} & \textbf{Definition} & \textbf{Keywords} \\
\hline
Collection & The methods and purposes used by a service provider to get user data. & Collect, personal, identifiable, telephone, number, phone, telephone number, IP address, phone number, IP, mobile, email,
address, name, date of birth, birthday, age, account, credit card, location, username, password, contact, zip code, postal code,
mailing address, phone \\
\hline
Sharing& The methods third parties use to share or acquire user information. & Party, share, sell, disclose, company, advertiser, provider, partner, public, analytics, companies, organizations, businesses,
contractors, divulge, sell, law, legal, regulation, third party, transfer, service providers, marketing partners, subsidiaries,
disclosure, safe harbor \\
\hline
Purpose& The objectives and reasons behind collecting and using user data.&Ads, use, services, verifying, purpose, fraud, prevention, improve products, identification, promotions, personalize, advertising,
analytics\\
\hline
Access & If users may access, edit, or remove their information, and how. &Delete, profile, correct, account, change, update, section, access, removal, request, modify, edit, settings, preferences, accurate \\
\hline
Security & How user data is safeguarded. & Secure, security, safeguard, protect, compromise, encrypt, advertiser set, unauthorized, access, SSL, socket, socket layer,
encryption, restrict, fraud \\
\hline
Policy Change & Whether and how users will be informed of privacy policy changes. &  Change, change privacy, policy time, current, policy agreement, update privacy, update, notice \\
\hline
Do Not Track & Whether and how internet tracking and advertising using Do Not Track signals are handled. &Signal, track, track request, browser, disable, track setting, cookies, web beacons, IP address \\
\hline
Legislation & The legal frameworks that empower individuals to control the collection, usage, and distribution of their personal information by businesses and organizations. & GDPR, CCPA, General Data Protection Regulation \\
\hline
Choice & User's right to make decisions about how their personal data is collected, used, and shared by a service or platform. & Opt, unsubscribe, disable, choose, choice, consent, setting, option, wish, agree, opt-in, opt-out, subscribe, do not track \\
\hline
Retention &The policies and practices related to the storage, archiving, and deletion of user data   &Retain, store, delete, deletion, database, participate, promotion, send friend, record, remove, retention, keep, data, backup,\\
\hline

IoT Data & Information collected from IoT devices and related services. & sensor data, device data, environmental data, operational data, health metrics, location data, Bluetooth, Wi-Fi, NFC, Capacitive NFC, LTE, device communication, connected devices, smart devices, user commands, voice control, device settings, interaction logs, health data, fitness tracking, biometric identifiers, heart rate, proximity data, ambient conditions, temperature, lighting, microphone, Barometer, cross-device tracking, RFID, Vibration sensor, Radar sensor, Pressure sensors, Ultrasonic sensors, Infrared sensors, RF sensor \\
\hline
\end{tabularx}
\caption{Privacy attributes extracted from a privacy policy based on keywords.}
\label{tab:privacy_keywords}
\end{table*}

\paragraph{Last Update.}
Policy updates are crucial to keeping users
informed about changes in the handling of their data. \system identifies 
% using an NLP technique, 
explicit mentions to the date in which the privacy policy was updated.

\paragraph{Regulations Compliance.}
Over 150 countries around the world have adopted new data protection regulations~\cite{banisar2023national}. An automated cross-country and manufacturer-wise assessment of regulatory compliance is essential for analyzing the policy landscape. \system employs a deep learning approach, utilizing the Bidirectional Encoder Representations of Transformers (BERT) model~\cite{2019}, fine-tuned on the Semantic Textual Similarity Benchmark dataset (STS-B)~\cite{cer-etal-2017-semeval}, to evaluate the changes in IoT device privacy policies before and after specific regulations (e.g., GDPR) came into effect. This approach generates a semantic similarity score between policy pairs (i.e., the policy before and after certain event), providing a numeric gauge of the policy changes. 

\paragraph{Overall Assessment.} \system summarizes the results of its privacy analysis of an IoT policy into an overall assessment (i.e., \textit{acceptable} or \textit{unacceptable}) inspired by the Mozilla Privacy Not Included (PNI) project~\cite{mozilla_privacy_not_included}. To this end, we created a dataset consisting of the 172 IoT devices analyzed by PNI (at the time of writing this paper). We partitioned the dataset into an 80\% training set (138 policies) and a 20\% testing set (34 policies). Notably, the dataset was imbalanced, with "acceptable" instances numbering 135 and "unacceptable" ones only 17. To address this, we employed random oversampling, effectively balancing the "unacceptable" class. We use the logistic regression classifier which estimates the probability of an outcome based on independent variables. This model is particularly effective for categorical target variables, such as policy categorization\cite{hosmer2013applied}. We considered 19 features that include the ones described above along with the features about readability that we will explain next. To optimize the model further, we used GridSearchCV from the \textit{sci-kit-learn}\footnote{\url{https://scikit-learn.org/}} library for hyperparameter tuning, ultimately enhancing the performance of our logistic regression model. 

\subsection{Readability Analysis}

\system extracts the following eight features as a result of an analysis of the readability of the policy.

\paragraph{Entropy.} In the realm of privacy policy analysis, entropy serves as a critical metric, offering a quantitative measure of the policy's textual uncertainty and complexity, thereby shedding light on interpretive challenges that users may face. The entropy of a language is a statistical quantity that measures how much information is generated on average for each letter in a text in that language. Hence, it defines the uncertainty or disorder in a text document.  Shannon~\cite{shannon1951prediction} presented a technique to calculate the entropy of English text using the following equation:
% arguing that everyone who speaks the language is well aware of the characteristics of the language. The uncertainty of the meaning of textual terms is expressed in two ways: the meaning we get from it and the context in which it is utilized. The equation for generating the entropy is given by:
\begin{equation} H(X) = -\sum_{i=1}^{n} P_{i} \log_{2}(P_{i})
\label{eq:entropy}
\end{equation}
\noindent where $H(X)$ represents the entropy of a discrete random variable X and $P_i$, is the probability of the ith outcome of the random variable X.
\system computes the entropy of a document  based on Equation~\ref{eq:entropy} by iterating over each word and noting its frequency of occurrence. Then, it divides the frequency by the total number of words to get an estimate of the probability of each word. Next, it calculates the average length of each word in bits by multiplying its probability by the negative logarithm (base 2) of that same probability. The entropy of the document is then the sum of these calculated values for all words.

\paragraph{Reading Time.} Privacy policies are hard to read and therefore do not help customers make informed decisions due to the fact that they are very lengthy and time-consuming~\cite{mcdonald2008cost}. Reading time is calculated using an individual's typical reading pace (roughly 238 WPM)~\cite{brysbaert2019many}. \system counts all the words in the document and divides the total by 238 to compute the estimated number of minutes that it would take a person to read the full privacy policy. 

\paragraph{Unique Words.} Privacy policies tend to use technical jargon to convey data usage and control to consumers. Unique, low-frequency words are crucial to understanding these documents, as they provide key context and learning aspects~\cite{hiebertunique}. Despite their scarcity, they make comprehension challenging, as understanding the content fully requires a strong grasp of this specialized vocabulary. 
% Interestingly, a narrow set of approximately 10,000 words, derived from 4,000 simple word families, makes up 90\% of text words~\cite{hiebert2012teaching}. 

The process begins by converting the text to lowercase and eliminating stop words, punctuation, and numbers followed by  standardized through tokenization~\cite{geitgey2018natural} using the Spacy library~\cite{spacy2}. Following standardization, the \system proceeds to identify unique words, which are words that have distinct character sequences. These unique words are counted, providing a distinct vocabulary size. Furthermore, the system calculates the ratio of the unique word count to the total word count in the document, offering a quantitative measure of the text's lexical diversity.


\paragraph{Coherence Score.} 
Topic modeling employs a coherence score to measure how well a topic is understood by people, as established by Syed et al.~\cite{syed2017full}. It evaluates word similarity within a topic based on their frequency in a document. The Latent Dirichlet Allocation (LDA) technique, a type of unsupervised machine learning, aids in text analysis by identifying the best topics to represent the data (Yu et al., 2001)~\cite{yu2001direct}. In this approach, a Dirichlet distribution is created first for documents in the subject space, and topics and words are selected from multinomial distributions. The coherence score, calculated as the sum of scores between every pair of words, is used to gauge the quality of the topics learned. The measure used in this case is CV, which computes scores via cosine similarity and normalized pointwise mutual information (NPMI) based on word co-occurrences. Then, the overall coherence of the privacy policy is computed as $\sum_{i < j} \text{score}(w_i, w_j)$, 


\noindent Where $w_i $and $w_j$ represent words at positions i and j respectively within a given text. In the context of readability, a high coherence score suggests a well-structured and clear flow of ideas, thereby increasing readability, while a low coherence score often indicates a disjointed or unclear progression of thoughts, potentially making the text more difficult to understand.
\paragraph{Frequency of Imprecise Words.}
Imprecise words, such as "commonly" or "normally" can create ambiguity, making it hard to understand a service provider's operations.
\system employs NLTK to tokenize the text and regex to count the frequency of imprecise words to measure their prevalence in the privacy policy. \Cref{table2} shows the list of imprecise words considered.

\paragraph{Connective Words Frequency.}
While connective words (such as "and" or "then") are useful to create coherent sentences, their overuse can make the text complex. 
% For instance, in this policy excerpt: "Our service, like many others, collects information. This typically includes data from online services, portable devices, cloud services, such as the internet browser, Source IP, unique device identifiers, language preference, referring site, the date and time of access, operating system, and mobile network information.", the conjunction "and" is excessively used, making the sentence complicated. 
\system, in a similar way than for the previous feature, counts the frequency of connective words using the list of words in \Cref{conn}.

\paragraph{Grammatical Errors.}
The integrity of a work depends on proper grammar, much as it does on word spelling~\cite{naber2003rule}.\system takes privacy document as input and then uses the NLTK library for tokenization (i.e., breaking the text into sentences) and the \texttt{language\_tool\_python} library to check for grammatical errors. It counts the total number of sentences and the number of sentences that contain at least one mistake providing a measure of the grammatical correctness of the input text.

\paragraph{Readability.} Readability signifies how easily a text, like a policy, can be understood, based on its vocabulary, syntax, and sentence structure. Various readability tests exist ~\cite{kouame2010using}, devised by linguists, each considering different text aspects. In our study, we employed the Flesch-Kincaid Grade Level ~\cite{flesch2007flesch}, which presents the score as a U.S. grade level. This metric represents the educational level required to understand a text and is computed using the following formula:
\begin{equation} \label{eq1}
\resizebox{0.9\hsize}{!}{$FKGL = 0.39 \left(\frac {total words}{total sentences}\right) + 11.8 \left(\frac {total syllables}{total words}\right) - 15.59$}
\end{equation}

\noindent In the Flesch-Kincaid Grade Level (FKGL) formula, 0.39 and 11.8 are weights for the average sentence length and syllables per word respectively. The constant -15.59 calibrates the score to U.S. grade levels.


\paragraph{Ambiguity.} 
While privacy policies should clearly state the data handling practices, privacy policies often contain ambiguous language~\cite{reidenberg2016ambiguity}. \system incorporates the supervised learning approach to classify a privacy policy based on a scale with three ambiguity levels (\textit{not ambiguous}, \textit{somewhat ambiguous}, and \textit{very ambiguous}) presented in~\cite{kotal2021effect}. We annotated 100 IoT device policies extracted from \system and trained a random forest classifier~\cite{breiman2001random} and a logistic regression~\cite{hosmer2013applied} classifier. \system applies both classifiers to each privacy policy and stores their output labels.
% The random forest classifier is a method that uses an ensemble of classification trees, each constructed using bootstrap samples and random variable subsets for splitting. This technique effectively combines bagging and random variable selection to yield low-bias, low-variance trees, contributing to an overall model with low bias and variance. Logistic regression, on the other hand, is a statistical model used in machine learning for classification problems. It estimates the probability of an outcome based on one or more predictor (independent) variables.  This model is particularly useful when the target variable is categorical, as it is in our case of policy ambiguity categorization \cite{hosmer2013applied}.

% There are numerous methods for detecting ambiguity in Natural Language~\cite{10.1145/1377836,yadav2021comprehensive,Franz1996AutomaticAR,SCHANK1972552}.
% Different linguistic characteristics of a text that influence its ambiguity have been defined in previous research in other technical publications~\cite{Gnova2011AFT,9284268,RePEc:ucp:jlstud:doi:10.1086/688669}. 


==> evaluation.tex <==
In this section, we assess the effectiveness and performance of \system by conducting an evaluation of both its policy collection and analysis capabilities.

\subsection{Evaluating Policy Collection}

\paragraph{Current Privacy Policy Extraction.}
We assessed the quality of our web-scraped data from Amazon against manually validated ``truth'' values for each of the top 30 records in ten categories of smart devices (i.e., 300 total devices). Our initial evaluation is focused on two key aspects: extraction of manufacturers and websites of manufacturers. We used three metrics in our evaluation: F1 score, recall, and precision. \Cref{tab:collection_results} shows the results of the experiment. For the manufacturer data, we observed a high overall F1 score (0.98), recall (0.96), and precision (0.99). For the collection of the website URL, \system achieves also a high overall F1 score (0.95), recall (0.91), and precision (0.99). These results highlight that \system can accurately obtain information about IoT device manufacturers and their websites, which is required to find their privacy policies.


\begin{table}[ht]
\centering
\small
\begin{tabular}{lccc|ccc}
\hline
 & \multicolumn{3}{c|}{\textbf{Manufacturer Collection}} & \multicolumn{3}{c}{\textbf{Website Collection}} \\
\textbf{Category} & \textbf{Recall} & \textbf{Prec.} & \textbf{F1} & \textbf{Recall} & \textbf{Prec.} & \textbf{F1}\\
\hline
Sensor & 0.90 & 1.00 & 0.95 & 0.95 & 1.00 & 0.98 \\
Projector & 1.00 & 1.00 & 1.00 & 0.94 & 0.94 & 0.94 \\
Bulb & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
Speaker & 0.97 & 1.00 & 0.98 & 0.97 & 1.00 & 0.98 \\
Alarm & 0.97 & 1.00 & 0.98 & 0.89 & 1.00 & 0.94 \\
Camera & 0.97 & 1.00 & 0.98 & 0.85 & 1.00 & 0.92 \\
Scale & 0.90 & 1.00 & 0.95 & 0.92 & 1.00 & 0.96 \\
Watch & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
Lock & 0.97 & 1.00 & 0.98 & 0.88 & 1.00 & 0.93 \\
Tracking & 0.97 & 0.97 & 0.97 & 0.74 & 1.00 & 0.85 \\
\hline
Overall & 0.96 & 0.99 & 0.98 & 0.91 & 0.99 & 0.95 \\
\hline
\end{tabular}
\caption{Evaluation of the extraction of manufacturers (Manufacturer Collection) and their websites (Website Collection) for IoT devices.}
\label{tab:collection_results}
\end{table}



To assess the effectiveness of our method for filtering and identifying IoT products from the broader range of extracted products, we randomly picked 100 products from total extracted products and manually checked each one to see if it was an IoT device. This gave us a set of true answers. Then, we used our method to identify these same products as IoT or not, creating a set of predictions. We compared our predictions with the true answers to see how well our method worked. The key measure we used was the F1 score. Our method scored 0.88 on this scale, which is quite good. This high score means that our method is effective at correctly identifying IoT products, and it doesn't often mistake non-IoT products for IoT ones. 

To evaluate the collection of privacy policies by \system we randomly selected 100 extracted manufacturer websites from the previous step. Then, we manually identify the policy URL on each website and compare it to the policy URL automatically extracted by \system. The results show that \system exhibited strong performance, achieving an F1 score of 0.94 for locating URLs linked to privacy policies, and a 0.76 F1 score for extracting the policy text from the web pages associated with the extracted URLs. This indicates that the system is highly precise and accurate in its extraction capabilities. \system encountered difficulties when the privacy policy was either present in another child component that renders on performing an event, or the website had a special download option for the privacy policy, which would require specialized parsers for certain websites and would not scale. These results show that the web parsing technique in \system is a feasible method for collecting privacy policies.


\paragraph{Past Privacy Policy Extraction.}
In this experiment, we selected randomly another 100 manufacturers (and their associated websites) from the previous step making sure that the companies existed on or before 2020. Then, for each of them, we randomly select a date between 2020 and 2022 and use \system to automatically retrieve the archived version of the manufacturer's website on that date (if available). Our results indicate that \system was able to retrieve archived websites for 64\% of them. After manually analyzing these retrieved websites, we observed that 8\% of them pointed to empty homepages. This can be attributed to the snapshots taken by the Wayback Machine, which sometimes do not capture any information at all. Delving further into the results, \system was successful in finding the archived privacy policy on the archived website of 30 out of 64 (47\%) manufacturers. For the remaining manufacturers (44\%), the failures were due to the absence of a privacy link in the snapshot. The average distance between the queried snapshot date and the retrieved snapshot date was 87 days. 


\paragraph{Privacy Policy Cleaning.}
We evaluate \system' cleaning performance by manually cleaning 10 policies and automatically comparing the number of tokens that can be extracted from both automatic and manually cleaned policies. We use the \textit{punkt} tokenizer model from NLTK~\cite{bird2009} to break the policy text into individual tokens for comparison. The comparison results show that \system's automatic cleaning achieves high precision (0.94), recall (0.97), and F1-score (0.95), demonstrating its effectiveness in retaining essential information while removing unnecessary content from the privacy policy.


% \noindent\textbf{Metrics Calculation:}
% The token sets of the original and cleaned texts were compared to calculate the precision, recall, and F1 score. True positives (tp) were tokens shared by both texts. False positives (fp) and false negatives (fn) were tokens unique to the cleaned and original texts, respectively. Then, precision (tp / (tp + fp)) and recall (tp / (tp + fn)) were computed. The F1 score, which represents the overall performance, was 2 * (precision * recall) / (precision + recall) \cite{sokolova2006}.


\subsection{Evaluating Policy Analysis}

To evaluate the insights extracted from each privacy policy, we leveraged existing ground truth datasets from the literature. As there does not exist a human-annotated dataset of privacy policies for IoT devices, we choose datasets of privacy policies of websites that include annotations. The dataset in~\cite{kotal2021effect}, which is based on the OPP-115 dataset~\cite{peters2018deep}, contains annotations on grammatical errors, frequency of imprecise words, and connectivity words. Then, for the remaining features of \system's readability analysis, we annotate 10 policies of the OPP-115 using popular and free web-based resources: \textit{Readable}\footnote{\url{https://readable.com}} for readability, \textit{Planetcalc}\footnote{\url{https://planetcalc.com}} for entropy, and \textit{The Read Time}\footnote{\url{https://thereadtime.com/}} for reading time. We show the results next for each of the features.

W.r.t. \textbf{grammatical errors}, 
We followed the benchmark study's\cite{kotal2021effect} methodology for our comparative analysis. Despite the benchmark's range of results, we were able to compare our specific scores effectively. Our results for the policy with the least grammatical errors nearly aligned with their lowest range, with a negligible difference of -0.06. However, for the policy with the most errors, we observed a higher difference, exceeding their range by about +0.7. This indicates our grammatical error detection tool, \textit{language\_tool\_python}, has a stringent approach toward grammatical correctness. For \textbf{connective words} We compared our results with the general ranges provided in study\cite{kotal2021effect}. For the policy with the least connective words, the deviation is minuscule at 0.005, aligning our results closely with their lower range. With the policy utilizing the most connective words, our figures slightly exceed theirs by 0.016, still affirming the consistency between our method and the reported study. 
For \textbf{imprecise words} we also compared the use of imprecise words in policies with the ranges from study \cite{kotal2021effect}. In the policy with the most imprecise words, our results were slightly higher, with a small difference of 0.05. For the policy with the fewest imprecise words, our results were a bit lower, with a  difference of 0.09, still affirming the consistency between our method and the reported study.

Our Flesch-Kincaid \textbf{readability} scores closely matched those from Readable, indicating agreement between the methods.  For instance, RedOrbit's privacy policy, our score was 10.26 compared to Readables's 10.4, and for sci-news policy, our score was 9.4 while Readable's was 8.9. Scores for Uptodate and Earthkam were also similar, with our approach producing scores of 12.9 and 14.6, compared to Readable's 12.9 and 15.5, respectively. Overall, our results were consistent with those from readable.com, affirming the reliability of our approach.
\system's measure \textbf{entropy} between 4.1-4.2, shows a high consistency with Planetcalc's range of 4.1-4.3. Specifically, Redorbit's privacy policy scored 4.1 with our method, versus 4.2 with Planetcalc. For Earthkam, Uptodate, and Amazon, both our method and Planetcalc agreed on scores of 4.2, with the exception of Amazon, where Planetcalc reported a slightly higher score of 4.3. This close alignment affirms the precision and reliability of our method.
In evaluating ten policies, our method calculated a total \textbf{reading time} of 120 minutes and 5 seconds, closely matching The Read Time's estimate of 120 minutes and 40 seconds. The small variance of 120 seconds between both methods underscores the precision of our evaluation technique. The \textbf{unique words}, \textbf{keyword usage}, and \textbf{last update} features are based on searching specific keywords in the document and the search function is a well-tested Python library.

Next, we evaluate the performance of the \textbf{ambiguity} feature. The results in \Cref{tab:amb} show that the classification of policy texts is significantly more challenging for more ambiguous policies. We observed a decrease in the F1 score from 86\% to 67\% as the ambiguity of the policy increased. Additionally, in the case of logistic regression, we observed that the F1 score dropped from 77\% to 69\% when moving from non-ambiguous to ambiguous policies. These findings indicate that classification algorithms have less accurate results for highly ambiguous policies.  This can be attributed to the fact that highly ambiguous policies have less well-defined requirements and guidelines, making it harder for classification algorithms to accurately assess them.

\begin{table}[!htb]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Ambiguity Class} & \textbf{Number of Policies} & \textbf{Random Forest Classifier} & \textbf{Logistic Regression} \\
\hline
Not Ambiguous & 283 & 0.86 & 0.77 \\
\hline
Somewhat Ambiguous & 90 & 0.67 & 0.72 \\
\hline
Very Ambiguous & 89 & 0.67 & 0.69 \\
\hline
\end{tabular}
}
\caption{F1-score of ambiguity determination models.}
\label{tab:amb}
\end{table}

% \textbf{Coherence.} Using the Latent Dirichlet Allocation (LDA) method through the Textacy library, we performed topic modelling on Bible data - mirroring the approach of Garbhapu and Bodapati. Our preprocessing and TF-IDF modelling produced a coherence score of 0.54, which aligned closely with their score of 0.58\cite{Garbhapu2020ACA}, validating our methodology.

Finally, we evaluate the performance of the classifier trained to predict a human analyst \textbf{overall assessment} using the subset of 172 privacy policies corresponding to devices analyzed by the Mozilla PNI initiative (with their corresponding human analyst assessment). We applied cross-validation for a reliable estimate of the model's effectiveness. The results (see \Cref{table:performance_metrics}) show that \system successfully predicts the human analyst assessment with a high F1-Score (0.91). \system performs better for the ``acceptable'' label than for the ``unacceptable'' label. This is due to the scarcity of unacceptable instances in the dataset which leads to low prediction accuracy, due to model bias and difficulty distinguishing this minority class despite using random oversampling. \Cref{fig:feat_imp} shows the importance of analysis of the different features used to train the model. Positive feature importance coefficient means the model's prediction accuracy increases with the feature value, while a negative one means the prediction accuracy decreases, assuming other features are constant. The results show that, in general, the features related to the privacy analysis tend to have a higher impact on the prediction than those related to readability. However, features like reading level, unique words, and reading time, score high importance which might indicate that the analyst's assessment is influenced by how much effort it requires to understand the policy. We would also like to highlight that PrivacyLens, matching the manual analysis of Mozilla PNI that took thousands of hours, showcases its proficiency in analyzing IoT device privacy policies.

\begin{table}[!htb]
\centering
\small
\begin{tabular}{l|c|c|c}
\hline
\textbf{Class} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} \\ \hline
acceptable        & 0.96               & 0.96            & 0.96             \\
unacceptable        & 0.67               & 0.67            & 0.67             \\ \hline
Weighted Avg  &     0.92    &  0.90  &    0.91 \\
\hline
\end{tabular}
\caption{Performance of the "overall assessment" model.}
\label{table:performance_metrics}
\end{table}

\begin{figure}[!htb]
  \centering
  \includegraphics[width=1\linewidth,height=4cm,scale=2]{feat_imp.jpg}
  \caption{Feature Importance of the "overall assessment" model.}
  \label{fig:feat_imp}
\end{figure}




% \subsection{Keyword Extraction Evaluation}

% Using the OPP-115 dataset, we scrutinized 10 randomly selected privacy policies to test our Python-based keyword extraction technique. In this manual process, we diligently identified and classified keywords into defined clusters, notably "Do Not Track" and "Opt-Out." We quantified the occurrence of each keyword, systematically compiling these data. Concentrating on the "Do Not Track" and "Opt-Out" categories served as a representative sample, illustrating the process and accuracy of our overall approach. Our method demonstrated remarkable accuracy, mirroring the precision of manual keyword extraction, thereby validating its efficacy. This result suggests that our technique offers a robust and reliable solution for extracting and categorizing critical terms from privacy policies, offering potential applications such as tracking policy shifts and improving user comprehension.


==> overview.tex <==

\system automatically and periodically collects and analyzes the privacy policies of IoT devices, including products such as smart home devices and wearable technology. 
In this section, we first present motivating use case scenarios supported by \system. Then, we overview the high-level architecture of the framework and its main components.

\paragraph{Motivating use cases.}
\system can enable different stakeholders to perform further analysis, such as:

\begin{figure*}[!htb]
\centering
\includegraphics[width=1\linewidth,scale=1.5]{Archit.png}
\caption{A high-level overview of \system. }
\label{fig:architecture}
\end{figure*}



\begin{itemize}
    \item \textit{IoT customers} can understand how their personal data will be collected, used, and protected by the smart device. Using \system, they can evaluate whether the device functionalities align with their privacy preferences and determine whether the privacy protection mechanisms implemented are sufficient. The comparison of insights for different devices of the same category (e.g., smart watches), or even of the same manufacturer (e.g., Fitbit) over the years, empowers customers to choose devices from manufacturers that prioritize privacy and security.
    % ultimately safeguarding their personal information and ensuring they make choices that align with their privacy needs and values.
    \item \textit{Product privacy lawyers} can compare their product's policy and ensure that it meets the industry best practices/standards and expectations of consumers.
    \system allows them to examine the strengths and weaknesses of competitor policies, identify areas for improvement or differentiation, and adopt better privacy protection mechanisms or create a privacy policy that can more easily be understood by the customers.
    \item \textit{Data protection regulators} can evaluate the influence of data protection regulations on various smart device manufacturers. \system offers insights into the changes instigated by these laws, shedding light on whether companies adapted their policies, as well as the timeline involved in such adaptations. By filling in these gaps, data protection regulators can also understand the trends in privacy policy updates, enabling more informed decision-making for future regulations.
\end{itemize}


\Cref{fig:architecture} shows an overview of the \system framework that can support these use cases, as well as others. The system and the data it generated can be accessed at \url{https://privacy-lens.web.app/home}\footnote{The source code of the system is available at \textit{URL removed for anonymization of the manuscript}.}. The framework is structured around three stages:

\paragraph{Collection.} \system finds and collects IoT device privacy policies from prominent e-commerce platforms (such as Walmart and Amazon), processes the documents extracted, and stores the information in a database. The input for this task is a list of 24 categories of smart IoT devices (e.g., smart cameras, lights, TVs, etc.) and the output is a cleaned and structured database of IoT device privacy policies. This output includes both current and past policies (extracted from a web archive) to enable the longitudinal study of IoT device privacy. We describe the methodology used to collect privacy policies in detail in \Cref{sect:extraction}. 
% To assess any changes in the privacy policies of the manufacturers due to the regulatory changes, we decided to collect and assess the past privacy policies of the manufacturers already collected. This allows us to assess any changes in the privacy policies of the manufacturers due to these regulatory changes. 

\paragraph{Analysis.} \system enables a comprehensive analysis of the database of IoT device privacy policies, focusing on two key aspects: textual analysis and privacy analysis. The goal of this stage is to generate metadata that enables different stakeholders to gain deeper insights into the privacy landscape of smart devices. The input is the cleaned and structured privacy policy data from the collection stage, and the output consists of metadata and in-depth analysis of similarity, ambiguity, keywords, and privacy insights. Further details on the analysis stage can be found in \Cref{sect:analysis}.
The results of these analyses are presented using a variety of exploratory tools, allowing stakeholders to synthesize complex data, draw meaningful conclusions, and develop targeted strategies to address privacy challenges more effectively. 

\paragraph{Publication.} The results from the analysis stage are published on a dedicated website, which is regularly updated every month. This update frequency ensures that users are always presented with the most current and accurate data available. In addition to the metadata, the raw data collected is also published for the purpose of transparency. \ref{fig:architecture} includes a representative screenshot of our website, showcasing its user-friendly interface and various sections, including but not limited to raw data, analysis results, and weekly updates. By making this wealth of information accessible and actionable, PrivacyLens contributes to the fostering of a more transparent and responsible digital ecosystem.
